Detection and Prediction of Nutrient Deficiency Stress using Longitudinal Aerial Imagery

Early, precise detection of nutrient deficiency stress (NDS) has key economic as well as environmental impact; precision application of chemicals in place of blanket application reduces operational costs for the growers while reducing the amount of chemicals which may enter the environment unnecessarily. Furthermore, earlier treatment reduces the amount of loss and therefore boosts crop production during a given season. With this in mind, we collect sequences of high-resolution aerial imagery and construct semantic segmentation models to detect and predict NDS across the field. Our work sits at the intersection of agriculture, remote sensing, and modern computer vision and deep learning. First, we establish a baseline for full-field detection of NDS and quantify the impact of pretraining, backbone architecture, input representation, and sampling strategy. We then quantify the amount of information available at different points in the season by building a single-timestamp model based on a UNet. Next, we construct our proposed spatiotemporal architecture, which combines a UNet with a convolutional LSTM layer, to accurately detect regions of the field showing NDS; this approach has an impressive IOU score of 0.53. Finally, we show that this architecture can be trained to predict regions of the field which are expected to show NDS in a later flight -- potentially more than three weeks in the future -- maintaining an IOU score of 0.47-0.51 depending on how far in advance the prediction is made. We will also release a dataset which we believe will benefit the computer vision, remote sensing, as well as agriculture fields. This work contributes to the recent developments in deep learning for remote sensing and agriculture, while addressing a key social challenge with implications for economics and sustainability.

==> aaai_formatting/criteria.tex <==
Significance of the problem
4. The social impact problem considered by this paper is significant and has not been adequately addressed by the AI community.
3. This paper represents a new take on a significant social impact problem that has been considered in the AI community before
2. The social impact problem considered by this paper has some significance and this paper represents a new take on the problem
1. This paper’s contribution was elsewhere: it follows up on an existing problem formulation or introduces a new problem with limited immediate potential for social impact

 
Engagement with literature
4. Shows an excellent understanding of other literature on the problem, including that outside computer science
3. Shows a strong understanding of other literature on the problem, perhaps focusing on various subtopics or on the CS literature
2. Shows a moderate understanding of other literature on the topic, but does not engage in depth
1. Does not engage sufficiently with other literature on the topic

 
Novelty of approach
4. Introduces a new model, data gathering technique, algorithm, and/or data analysis technique
3. Substantially improves upon an existing model, data gathering technique, algorithm, and/or data analysis technique
2. Makes a moderate improvement to an existing model, data gathering technique, algorithm, and/or data analysis technique
1. This paper’s contribution was elsewhere: it employs existing models, data gathering techniques, algorithms, and/or data analysis technique (e.g., the paper presents a new experimental design and evaluation procedure).

Justification of approach
4. Thoroughly and convincingly justifies the approach taken, explaining strengths and weaknesses as compared to other alternatives
3. The justification of the approach is convincing overall, but could have been more thorough and/or alternatives could have been considered in more detail
2. The justification of the approach is relatively convincing, but has weaknesses
1. The justification of the approach is flawed and/or not convincing

Quality of evaluation
4. Evaluation was exemplary: data described the real world and was analyzed thoroughly
3. Evaluation was convincing: datasets were realistic; analysis was solid
2. Evaluation was adequate, but had significant flaws: datasets were unrealistic and/or analysis was insufficient
1. Evaluation was unconvincing

 
Facilitation of follow-up work
4. Excellent facilitation of follow-up work: open-source code; public datasets; and a very clear description of how to use these elements in practice
3. Strong facilitation of follow-up work: some elements are shared publicly (data, code, or a running system) and little effort would be required to replicate the results or apply them to a new domain
2. Adequate facilitation of follow-up work: moderate effort would be required to replicate the results or apply them to a new domain
1. Weak facilitation of follow-up work: considerable effort would be required to replicate the results or apply them to a new domain

 
Scope and promise for social impact
4. Likelihood of social impact is extremely high: the paper’s ideas are already being used in practice or could be immediately
3. Likelihood of social impact is high: relatively little effort would be required to put this paper’s ideas into practice, at least for a pilot study
2. Likelihood of social impact is moderate: this paper gets us closer to its goal, but considerably more work would be required before the paper’s ideas could be implemented in practice
1. Likelihood of social impact is low: the ideas proposed in this paper are unlikely to make a significant impact on the proposed problem
